Hyperbolic Active Learning for Semantic Segmentation under Domain Shift

We introduce a hyperbolic neural network approach to pixel-level active learning for semantic segmentation. Analysis of the data statistics leads to a novel interpretation of the hyperbolic radius as an indicator of data scarcity. In HALO (Hyperbolic Active Learning Optimization), for the first time, we propose the use of epistemic uncertainty as a data acquisition strategy, following the intuition of selecting data points that are the least known. The hyperbolic radius, complemented by the widely-adopted prediction entropy, effectively approximates epistemic uncertainty. We perform extensive experimental analysis based on two established synthetic-to-real benchmarks, i.e. GTAV $\rightarrow$ Cityscapes and SYNTHIA $\rightarrow$ Cityscapes. Additionally, we test HALO on Cityscape $\rightarrow$ ACDC for domain adaptation under adverse weather conditions, and we benchmark both convolutional and attention-based backbones. HALO sets a new state-of-the-art in active learning for semantic segmentation under domain shift and it is the first active learning approach that surpasses the performance of supervised domain adaptation while using only a small portion of labels (i.e., 1%).

==> figures/entropy_corr.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/supplementary/entropy_corr.jpeg}
\caption{(left) Plot of average per-class entropy Vs. class accuracies; (right) Plot of average per-class entropy Vs. the percentage of per-class target pixels. Zoom in for the details. 
}
\label{fig:entropy_corr}
\end{figure}


==> figures/pipeline.tex <==
\begin{figure*}[t]
    \begin{minipage}{.1\linewidth}
    \centering
    \includegraphics[trim={0 4cm 4cm 7cm}, scale=0.21]{figures/images/pipeline.pdf}
    \label{fig:pipeline}
    \end{minipage}
\caption{pipeline}
%\vspace{-0.4cm}
\label{fig:pipeline}
\end{figure*}

==> figures/var_mod_evolution.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/supplementary/variance_selected_pixel.png}
\caption{Evolution of the variance (y axis) of selected pixel distributions with varying budget (x axis).}
\label{fig:var_mod_evolution}
\end{figure}


==> tables/ablation.tex <==
\begin{table}[t]
% \begin{wraptable}{r}{0.6\textwidth}
\centering
\caption{\textbf{Ablation study on GTAV $\rightarrow$ CS.} The table showcases the results of our ablation study conducted with the Hyperbolic DeepLab-v3+ as backbone, on the source$+$target protocol with $5\%$ of labels. We explore various selection criteria, number of quantization sub-intervals, and region sizes to analyze their impact on performance.}
\label{tab:main-ablation}
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{clcc}
\toprule
\multirow{2}{*}{\centering \textbf{Method}} & \multirow{2}{*}{\centering \textbf{Selection Criteria}} & \textbf{Region} & \multirow{2}{*}{\centering \textbf{mIoU}} \\
& & \textbf{Size} & \\
\midrule
(a) & Hyper Boundaries only & $5\times 5$ & 63.4 \\
(b) & Impurity only & $5\times 5$ & 56.6 \\
(c) & Entropy only & $5\times 5$ & 63.2 \\
(d) & Impurity $+$ Entropy & $5\times 5$ & 73.0 \\
(e) & \ub{Hyper Boundaries $+$ Entropy} & \ub{$\mathbf{5\times 5}$} & \ub{74.1} \\
% \midrule
% \checkmark && \checkmark & 10 & 5 & 73.5 \\
% \checkmark && \checkmark & 50 & 5 & 73.6 \\
% \checkmark && \checkmark & 200 & 5 & 73.9 \\
% \midrule
(f) & Hyper Boundaries $+$ Entropy & $3\times 3$ & 73.8 \\
(g) & Hyper Boundaries $+$ Entropy & $7\times 7$ & 73.7 \\
\bottomrule
\end{tabular}%
}
% \end{wraptable}
\end{table}
% \vspace{-10pt}

==> tables/ablation_tables_minipages.tex <==
\begin{table}[t]
% \caption{\textbf{Ablation study on GTAV $\rightarrow$ CS.} a) results of our ablation study conducted with the Hyperbolic DeepLab-v3+ as backbone, on the source$+$target protocol with $5\%$ of labels. We explore various selection criteria and region sizes to analyze their impact on performance. b) HALO performance on the \textbf{source-free protocol} in comparison with previous approaches.} 
% \label{fig:figure_table}
\begin{minipage}{0.40\linewidth}
\centering
\caption{HALO performance on the \textbf{source-free protocol} compared with previous UDA and ADA approaches.}
\vspace{5pt}
\label{tab:source-free}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc}
\toprule
\textbf{Method} & \textbf{Budget} & \textbf{mIoU} \\
\midrule
URMA \citep{teja2021uncertainty} & - & 45.1 \\
LD \citep{you21} & - & 45.5 \\
SFDA \citep{Kundu_2021_ICCV} & - & 53.4 \\
\midrule
RIPU \citep{xie2022ripu} & 2.2\% & 67.1 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO} (ours) & 2.2\% & \textbf{70.1} \\
\midrule
\rowcolor[HTML]{ebebeb}
\textbf{HALO}$^\sharp$ (ours) & 5\% & \textbf{73.3} \\
\bottomrule
\end{tabular}%
}
\end{minipage}
\hfill
\begin{minipage}{0.50\linewidth}
\centering
\caption{Ablation study conducted with the Hyperbolic DeepLab-v3+ as backbone on the source$+$target protocol with $5\%$ budget. Performance of entropy and hyperbolic radius scores in isolation (a and b) and combined (c).}
\label{tab:main-ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc}
\toprule
\textbf{Ablative version} & \textbf{mIoU} \\
\midrule
(a)\, Entropy only & 63.2 \\
(b)\, Hyperbolic Radius only & 64.1 \\
(c)\, \textbf{Hyperbolic Radius $\odot$ Entropy (HALO)} & \textbf{74.5} \\
\bottomrule
\end{tabular}%
}
\end{minipage}
% \vspace{-0.4cm}
\end{table}

==> tables/cityscapes-acdc.tex <==
%%%%%%% ACDC

\begin{table*}[t]
\caption{Comparison of mIoU results for HALO (ours) and RIPU \citep{xie2022ripu} on the \textbf{Cityscapes$\rightarrow$ACDC} task. Methods marked with $^\sharp$ are based on DeepLab-v3+ \citep{chen2018encoderdecoder}, whereas all the others use DeepLab-v2 \citep{deeplab2018}.}
\label{tab:acdc}
\centering
\begin{sc}
\begin{small}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccccccccc}
\toprule
Method & \rot{road} & \rot{side.} & \rot{buil.} & \rot{wall} & \rot{fence} & \rot{pole} & \rot{light} & \rot{sign} & \rot{veg.} & \rot{terr.} & \rot{sky} & \rot{pers.} & \rot{rider} & \rot{car} & \rot{truck} & \rot{bus} & \rot{train} & \rot{motor.} & \rot{bike} & mIoU \\
\midrule
RIPU (2.2\%) & 91.4 & 69.5 & 83.8 & \textbf{52.7} & 41.6 & 52.8 & 66.4 & 54.2 & \textbf{85.1} & 47.5 & \textbf{94.7} & 54.5 & 21.8 & \textbf{85.5} & \textbf{58.7} & 58.8 & \textbf{76.9} & 41.4 & \textbf{45.9} & 62.3 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO (2.2\%)} & \textbf{92.6} & \textbf{71.3} & \textbf{84.5} & 51.3 & \textbf{43.1} & \textbf{53.5} & \textbf{67.2} & \textbf{57.6} & 85.1 & \textbf{49.5} & 94.5 & \textbf{57.2} & \textbf{28.6} & 84.1 & 53.3 & \textbf{76.0} & 66.9 & \textbf{44.1} & 41.4 & \textbf{63.2} \\
\midrule
RIPU (5\%)$^\sharp$ & \textbf{92.7} & \textbf{72.5} & 84.7 & 53.1 & 44.8 & 56.7 & 69.1 & 58.9 & 85.9 & 46.9 & \textbf{95.3} & 57.2 & 24.3 & 84.5 & \textbf{61.4} & 59.4 & 79.0 & 36.9 & 43.6 & 63.5 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO (5\%)}$^\sharp$ & 92.6 & 72.2 & \textbf{84.8} & \textbf{54.9} & \textbf{47.7} & \textbf{59.5} & \textbf{71.5} & \textbf{61.1} & \textbf{86.1} & \textbf{49.5} & 95.2 & \textbf{60.7} & \textbf{30.6} & \textbf{85.8} & 58.4 & \textbf{73.8} & \textbf{82.0} & \textbf{41.6} & \textbf{53.2} & \textbf{66.4} \\
\bottomrule
\end{tabular}%
}
\end{small}
\end{sc}
\end{table*}

==> tables/embeddings.tex <==
\begin{table}[ht]
\centering
\caption{Performance comparison of Euclidean and hyperbolic models with varying output channels (10, 64, and 512) in source-only and source$+$target protocols.
% The Hyperbolic DeepLab-v3+ model demonstrates superior performance in lower channel versions, while HALO exhibits robustness across different channel sizes.
}
\label{tab:embeddings}
\begin{tabular}{lccc}
\toprule
Encoder & Protocol & Channels & mIoU (\%) \\
\midrule
DeepLab-v3+ & source-only & 10 & 37.3 \\
DeepLab-v3+ & source-only & 64 & 37.9 \\
DeepLab-v3+ & source-only & 512 & 36.3 \\
Hyper DeepLab-v3+ & source-only & 10 & 39.7 \\
Hyper DeepLab-v3+ & source-only & 64 & 38.9 \\
Hyper DeepLab-v3+ & source-only & 512 & 35.9 \\
\midrule
RIPU \cite{xie2022ripu} & source$+$target & 10 & 72.3 \\
RIPU \cite{xie2022ripu} & source$+$target & 64 & 72.0 \\
RIPU \cite{xie2022ripu} & source$+$target & 512 & 71.2 \\
HALO & source$+$target & 10 & 73.8 \\
\ub{HALO} & \ub{source$+$target} & \ub{64} & \ub{74.1} \\
HALO & source$+$target & 512 & 73.7 \\
\bottomrule
\end{tabular}
\end{table}

% HALO w/o HFR & source-only & 10 & 26.8 \\
% HALO w/o HFR & source-only & 64 & 33.1 \\
% HALO w/o HFR & source-only & 256 & 19.5 \\


==> tables/gtav-cityscapes.tex <==
% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}


\begin{table*}[t]
\caption{Comparison of mIoU results for different methods on the \textbf{GTAV$\rightarrow$Cityscapes} task. Methods marked with $^\sharp$ are based on DeepLab-v3+ \citep{chen2018encoderdecoder}, the ones with $^\dagger$ on SegFormer-B4 \citep{xie2021segformer}, whereas all the others use DeepLab-v2 \citep{deeplab2018}.}
\label{tab:gtav-cityscapes}
\vskip 0.1in
\centering
\begin{sc}
\begin{small}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccccccccccc}
\toprule
Method & Budget & \rot{road} & \rot{side.} & \rot{buil.} & \rot{wall} & \rot{fence} & \rot{pole} & \rot{light} & \rot{sign} & \rot{veg.} & \rot{terr.} & \rot{sky} & \rot{pers.} & \rot{rider} & \rot{car} & \rot{truck} & \rot{bus} & \rot{train} & \rot{motor.} & \rot{bike} & mIoU \\
\midrule
Eucl. Source Only & 0\% & 75.8 & 16.8 & 77.2 & 12.5 & 21.0 & 25.5 & 30.1 & 20.1 & 81.3 & 24.6 & 70.3 & 53.8 & 26.4 & 49.9 & 17.2 & 25.9 & 6.5 & 25.3 & 36.0 & 36.6 \\
Hyper. Source Only & 0\% & 62.4 & 18.7 & 66.8 & 17.4 & 13.8 & 29.2 & 30.4 & 7.4 & 83.2 & 23.8 & 78.2 & 56.1 & 30.3 & 70.6 & 25.0 & 17.8 & 0.3 & 27.6 & 27.0 & 36.1 \\
Eucl. Source Only$^\sharp$ & 0\% & 73.4 & 19.7 & 79.2 & 31.5 & 10.7 & 27.1 & 26.3 & 13.0 & 81.5 & 30.0 & 78.9 & 53.4 & 26.3 & 69.5 & 22.0 & 20.4 & 13.4 & 25.7 & 18.9 & 37.9 \\
Hyper. Source Only$^\sharp$ & 0\% & 71.7 & 22.6 & 76.6 & 26.6 & 14.8 & 31.5 & 32.6 & 11.9 & 83.8 & 22.8 & 79.9 & 59.7 & 27.3 & 62.2 & 29.3 & 35.8 & 10.2 & 26.6 & 14.8 & 38.9 \\
Eucl. Source Only$^\dagger$ & 0\% & 88.9 & 35.2 & 83.5 & 37.2 & 24.8 & 34.3 & 47.8 & 29.5 & 86.7 & 31.5 & 84.9 & 61.0 & 31.7 & 84.6 & 46.0 & 47.9 & 33.5 & 34.5 & 37.0 & 50.5 \\
Hyper. Source Only$^\dagger$ & 0\% & 85.9 & 37.1 & 84.4 & 37.2 & 31.2 & 33.6 & 46.5 & 27.9 & 86.3 & 35.8 & 88.2 & 62.9 & 34.3 & 85.6 & 43.7 & 42.4 & 51.8 & 38.6 & 47.1 & 52.7 \\
\midrule
% CBST \citep{zou2018unsupervised} & 91.8 & 53.5 & 80.5 & 32.7 & 21.0 & 34.0 & 28.9 & 20.4 & 83.9 & 34.2 & 80.9 & 53.1 & 24.0 & 82.7 & 30.3 & 35.9 & 16.0 & 25.9 & 42.8 & 45.9 \\
% MRKLD \citep{Zou_2019_ICCV} & 91.0 & 55.4 & 80.0 & 33.7 & 21.4 & 37.3 & 32.9 & 24.5 & 85.0 & 34.1 & 80.8 & 57.7 & 24.6 & 84.1 & 27.8 & 30.1 & 26.9 & 26.0 & 42.3 & 47.1 \\
% Seg-Uncertainty \citep{zheng2021rectifying} & 90.4 & 31.2 & 85.1 & 36.9 & 25.6 & 37.5 & 48.8 & 48.5 & 85.3 & 34.8 & 81.1 & 64.4 & 36.8 & 86.3 & 34.9 & 52.2 & 1.7 & 29.0 & 44.6 & 50.3 \\
% TPLD \citep{shin2020two} & 94.2 & 60.5 & 82.8 & 36.6 & 16.6 & 39.3 & 29.0 & 25.5 & 85.6 & 44.9 & 84.4 & 60.6 & 27.4 & 84.1 & 37.0 & 47.0 & 31.2 & 36.1 & 50.3 & 51.2 \\
% DPL-Dual \citep{cheng2021dual} & 92.8 & 54.4 & 86.2 & 41.6 & 32.7 & 36.4 & 49.0 & 34.0 & 85.8 & 41.3 & 86.0 & 63.2 & 34.2 & 87.2 & 39.3 & 44.5 & 18.7 & 42.6 & 43.1 & 53.3 \\
% ProDA \citep{zhang2021prototypical} & 87.8 & 56.0 & 79.7 & 46.3 & 44.8 & 45.6 & 53.5 & 53.5 & 88.6 & 45.2 & 82.1 & 70.7 & 39.2 & 88.8 & 45.5 & 59.4 & 1.0 & 48.9 & 56.4 & 57.5 \\
% WeakDA (point) \citep{paul2020domain} & 94.0 & 62.7 & 86.3 & 36.5 & 32.8 & 38.4 & 44.9 & 51.0 & 86.1 & 43.4 & 87.7 & 66.4 & 36.5 & 87.9 & 44.1 & 58.8 & 23.2 & 35.6 & 55.9 & 56.4 \\
% \midrule
LabOR \citep{shin2021labor} & 2.2\% & 96.6 & 77.0 & 89.6 & 47.8 & 50.7 & \textbf{48.0} & \textbf{56.6} & 63.5 & 89.5 & 57.8 & 91.6 & 72.0 & 47.3 & 91.7 & 62.1 & 61.9 & 48.9 & 47.9 & 65.3 & 66.6 \\
RIPU \citep{xie2022ripu} & 2.2\% & 96.5 & 74.1 & 89.7 & 53.1 & 51.0 & 43.8 & 53.4 & 62.2 & 90.0 & 57.6 & 92.6 & 73.0 & 53.0 & \textbf{92.8} & 73.8 & \textbf{78.5} & 62.0 & \textbf{55.6} & 70.0 & 69.6 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO} (ours) & 2.2\% & \textbf{97.5} & \textbf{79.9} & \textbf{90.2} & \textbf{55.6} & \textbf{51.5} & 45.3 & 56.2 & \textbf{66.2} & \textbf{90.2} & \textbf{58.6} & \textbf{92.8} & \textbf{73.3} & \textbf{53.5} & 92.6 & \textbf{76.9} & 76.2 & \textbf{64.2} & 55.2 & \textbf{70.1} & \textbf{70.8} \\
\midrule
AADA$^\sharp$ \citep{su2020active} & 5\% & 92.2 & 59.9 & 87.3 & 36.4 & 45.7 & 46.1 & 50.6 & 59.5 & 88.3 & 44.0 & 90.2 & 69.7 & 38.2 & 90.0 & 55.3 & 45.1 & 32.0 & 32.6 & 62.9 & 59.3 \\
MADA$^\sharp$ \citep{ning2021multi} & 5\% & 95.1 & 69.8 & 88.5 & 43.3 & 48.7 & 45.7 & 53.3 & 59.2 & 89.1 & 46.7 & 91.5 & 73.9 & 50.1 & 91.2 & 60.6 & 56.9 & 48.4 & 51.6 & 68.7 & 64.9 \\
D$^2$ADA$^\sharp$ \citep{wu2022d2ada} & 5\% & 97.0 & 77.8 & 90.0 & 46.0 & \textbf{55.0} & 52.7 & 58.7 & 65.8 & 90.4 & 58.9 & 92.1 & 75.7 & 54.4 & 92.3 & 69.0 & 78.0 & 68.5 & 59.1 & 72.3 & 71.3 \\
RIPU$^\sharp$ \citep{xie2022ripu} & 5\% & 97.0 & 77.3 & 90.4 & \textbf{54.6} & 53.2 & 47.7 & 55.9 & 64.1 & 90.2 & 59.2 & 93.2 & 75.0 & 54.8 & 92.7 & 73.0 & 79.7 & 68.9 & 55.5 & 70.3 & 71.2 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO}$^\sharp$ (ours) & 5\% & \textbf{97.6} & \textbf{81.0} & \textbf{91.4} & 53.7 & 54.9 & \textbf{56.7} & \textbf{62.9} & \textbf{72.1} & \textbf{91.4} & \textbf{60.5} & \textbf{94.1} & \textbf{78.0} & \textbf{57.3} & \textbf{94.0} & \textbf{81.4} & \textbf{84.7} & \textbf{70.1} & \textbf{60.0} & \textbf{73.3} & \textbf{74.5} \\
\textbf{HALO}$^\dagger$ (ours) & 5\% & 98.2 & 85.4 & 92.5 & 62.5 & 61.6 & 58.3 & 67.7 & 74.9 & 92.2 & 65.1 & 94.7 & 79.9 & 60.8 & 94.6 & 84.1 & 85.4 & 83.6 & 61.2 & 75.5 & 77.8 \\
\midrule
Eucl. Supervised DA & 100\% & 96.8 & 77.5 & 90.0 & 53.5 & 51.5 & 47.6 & 55.6 & 62.9 & 90.2 & 58.2 & 92.3 & 73.7 & 52.3 & 92.4 & 74.3 & 77.1 & 64.5 & 52.4 & 70.1 & 70.2 \\
Hyper. Supervised DA & 100\% & 97.3 & 79.0 & 89.8 & 50.3 & 51.8 & 43.9 & 52.0 & 61.8 & 89.8 & 58.0 & 92.6 & 71.3 & 50.5 & 91.8 & 65.6 & 78.3 & 64.9 & 52.4 & 67.7 & 68.8 \\
Eucl. Supervised DA$^\sharp$ & 100\% & 97.4 & 77.9 & 91.1 & 54.9 & 53.7 & 51.9 & 57.9 & 64.7 & 91.1 & 57.8 & 93.2 & 74.7 & 54.8 & 93.6 & 76.4 & 79.3 & 67.8 & 55.6 & 71.3 & 71.9 \\
Hyper. Supervised DA$^\sharp$ & 100\% & 97.6 & 81.2 & 90.7 & 49.9 & 53.2 & 53.5 & 58.0 & 67.2 & 91.0 & 59.1 & 93.9 & 74.2 & 52.6 & 93.1 & 76.4 & 81.0 & 67.0 & 55.0 & 70.8 & 71.9 \\
Eucl. Supervised DA$^\dagger$ & 100\% &&&&&&&&&&&&&&&&&&&& X \\
Hyper. Supervised DA$^\dagger$ & 100\% & 98.2 & 85.0 & 92.4 & 61.5 & 59.6 & 57.9 & 65.8 & 73.3 & 92.1 & 64.4 & 94.7 & 78.9 & 59.2 & 94.4 & 82.8 & 83.5 & 78.1 & 61.0 & 74.7 & 76.7 \\
\bottomrule
\end{tabular}
}
\end{small}
\end{sc}
\end{table*}

==> tables/segformer-acdc.tex <==
\begin{table}[t]
\centering
\caption{Comparison of mIoU results of HALO using DeepLab-v3+ (dlv3+) and SegFormer-b4 (SF-b4) on the \textbf{Cityscapes $\rightarrow$ ACDC} adaptation task.}
\label{tab:segformer-acdc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
Method & \rot{road} & \rot{side.} & \rot{buil.} & \rot{wall} & \rot{fence} & \rot{pole} & \rot{light} & \rot{sign} & \rot{veg.} & \rot{terr.} & \rot{sky} & \rot{pers.} & \rot{rider} & \rot{car} & \rot{truck} & \rot{bus} & \rot{train} & \rot{motor.} & \rot{bike} & mIoU \\
\midrule
HALO (dlv3+) & 92.6 & 72.2 & 84.8 & 54.9 & 47.7 & 59.5 & 71.5 & 61.1 & 86.1 & 49.5 & 95.2 & 60.7 & \textbf{30.6} & 85.8 & 58.4 & 73.8 & 82.0 & 41.6 & 53.2 & 66.4 \\
\textbf{HALO (SF-b4)} & \textbf{95.2} & \textbf{79.8} & \textbf{88.2} & \textbf{60.2} & \textbf{51.1} & \textbf{64.1} & \textbf{78.2} & \textbf{65.6} & \textbf{87.9} & \textbf{55.7} & \textbf{95.5} & \textbf{66.3} & 20.7 & \textbf{88.9} & \textbf{82.2} & \textbf{89.3} & \textbf{87.9} & \textbf{50.4} & \textbf{59.0} & \textbf{71.9} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/segformer-gta.tex <==
\begin{table}[t]
\centering
\caption{Comparison of mIoU results of HALO using DeepLab-v2 (dlv2), DeepLab-v3+ (dlv3+) and SegFormer-b4 (SF-b4) on the \textbf{GTAV $\rightarrow$ Cityscapes} adaptation task.}
\label{tab:segformer-gta}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
Method & \rot{road} & \rot{side.} & \rot{buil.} & \rot{wall} & \rot{fence} & \rot{pole} & \rot{light} & \rot{sign} & \rot{veg.} & \rot{terr.} & \rot{sky} & \rot{pers.} & \rot{rider} & \rot{car} & \rot{truck} & \rot{bus} & \rot{train} & \rot{motor.} & \rot{bike} & mIoU \\
\midrule
Source Only (dlv2) & 62.4 & 18.7 & 66.8 & 17.4 & 13.8 & 29.2 & 30.4 & 7.4 & 83.2 & 23.8 & 78.2 & 56.1 & 30.3 & 70.6 & 25.0 & 17.8 & 0.3 & 27.6 & 27.0 & 36.1 \\
Source Only (dlv3+) & 71.7 & 22.6 & 76.6 & 26.6 & 14.8 & 31.5 & 32.6 & 11.9 & 83.8 & 22.8 & 79.9 & 59.7 & 27.3 & 62.2 & 29.3 & 35.8 & 10.2 & 26.6 & 14.8 & 38.9 \\
Source Only (SF-b4) & 85.9 & 37.1 & 84.4 & 37.2 & 31.2 & 33.6 & 46.5 & 27.9 & 86.3 & 35.8 & 88.2 & 62.9 & 34.3 & 85.6 & 43.7 & 42.4 & 51.8 & 38.6 & 47.1 & 52.7 \\
\midrule
HALO (5\%) (dlv3+) & 97.6 & 81.0 & 91.4 & 53.7 & 54.9 & 56.7 & 62.9 & 72.1 & 91.4 & 60.5 & 94.1 & 78.0 & 57.3 & 94.0 & 81.4 & 84.7 & 70.1 & 60.0 & 73.3 & 74.5 \\
\textbf{HALO (5\%) (SF-b4)} & \textbf{98.2} & \textbf{85.4} & \textbf{92.5} & \textbf{62.5} & \textbf{61.6} & \textbf{58.3} & \textbf{67.7} & \textbf{74.9} & \textbf{92.2} & \textbf{65.1} & \textbf{94.7} & \textbf{79.9} & \textbf{60.8} & \textbf{94.6} & \textbf{84.1} & \textbf{85.4} & \textbf{83.6} & \textbf{61.2} & \textbf{75.5} & \textbf{77.8} \\
\midrule
Supervised DA (dlv2) & 97.3 & 79.0 & 89.8 & 50.3 & 51.8 & 43.9 & 52.0 & 61.8 & 89.8 & 58.0 & 92.6 & 71.3 & 50.5 & 91.8 & 65.6 & 78.3 & 64.9 & 52.4 & 67.7 & 68.8 \\
Supervised DA (dlv3+) & 97.6 & 81.2 & 90.7 & 49.9 & 53.2 & 53.5 & 58.0 & 67.2 & 91.0 & 59.1 & 93.9 & 74.2 & 52.6 & 93.1 & 76.4 & 81.0 & 67.0 & 55.0 & 70.8 & 71.9 \\
Supervised DA (SF-b4) & 98.2 & 85.0 & 92.4 & 61.5 & 59.6 & 57.9 & 65.8 & 73.3 & 92.1 & 64.4 & 94.7 & 78.9 & 59.2 & 94.4 & 82.8 & 83.5 & 78.1 & 61.0 & 74.7 & 76.7 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/segformer-synthia.tex <==
\begin{table}[t]
\centering
\caption{Comparison of mIoU results of HALO using DeepLab-v2 (dlv2), DeepLab-v3+ (dlv3+) and SegFormer-b4 (SF-b4) on the \textbf{Synthia$\rightarrow$Cityscapes} adaptation task.}
\label{tab:segformer-synthia}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccc}
\toprule
Method & \rot{road} & \rot{side.} & \rot{buil.} & \rot{wall*} & \rot{fence*} & \rot{pole*} & \rot{light} & \rot{sign} & \rot{veg.} & \rot{sky} & \rot{pers.} & \rot{rider} & \rot{car} & \rot{bus} & \rot{motor.} & \rot{bike} & mIoU & mIoU* \\
\midrule
Source Only (dlv2) & 36.4 & 21.1 & 56.4 & 13.3 & 0.1 & 24.8 & 0.0 & 9.5 & 78.8 & 70.4 & 54.2 & 8.6 & 77.9 & 35.8 & 11.7 & 27.3 & 32.9 & 37.5 \\
Source Only (dlv3+) & 60.5 & 27.4 & 75.2 & 13.3 & 0.3 & 31.4 & 0.0 & 23.2 & 79.3 & 68.1 & 57.8 & 18.7 & 61.3 & 27.3 & 10.3 & 23.5 & 36.1 & 41.0 \\
Source Only (SF-b4) & 70.3 & 26.9 & 83.2 & 17.0 & 0.4 & 39.9 & 43.2 & 20.5 & 84.8 & 83.6 & 59.4 & 20.1 & 78.6 & 45.6 & 16.5 & 12.4 & 43.9 & 49.6 \\
\midrule
HALO (5\%) (dlv3+) & 97.5 & 81.5 & 91.5 & 56.5 & 52.7 & 57.0 & 63.2 & 72.9 & 92.0 & 94.4 & 77.8 & 57.4 & 94.4 & \textbf{86.1} & 60.5 & 73.5 & 75.6 & 80.2 \\
\textbf{HALO (5\%) (SF-b4)} & \textbf{98.3} & \textbf{86.5} & \textbf{92.6} & \textbf{61.0} & \textbf{61.5} & \textbf{60.6} & \textbf{67.6} & \textbf{76.2} & \textbf{93.2} & \textbf{94.6} & \textbf{80.8} & \textbf{58.9} & \textbf{95.0} & 85.1 & \textbf{62.7} & \textbf{75.6} & \textbf{78.1} & \textbf{82.1} \\
\midrule
Supervised DA (dlv2) & 97.6 & 81.9 & 90.2 & 52.0 & 49.6 & 45.5 & 51.7 & 65.0 & 90.9 & 93.0 & 73.1 & 50.3 & 92.6 & 80.7 & 50.8 & 69.2 & 70.9 & 75.9 \\
Supervised DA (dlv3+) & 97.7 & 82.2 & 90.3 & 53.0 & 48.8 & 51.7 & 56.0 & 66.1 & 91.4 & 94.2 & 75.0 & 51.5 & 93.4 & 82.1 & 52.8 & 70.2 & 72.3 & 77.1 \\
Supervised DA (SF-b4) & 98.3 & 86.6 & 92.7 & 61.3 & 61.1 & 60.7 & 66.5 & 75.5 & 93.1 & 94.7 & 80.2 & 57.7 & 95.0 & 86.2 & 60.3 & 74.9 & 77.8 & 81.7 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/synthia-cityscapes.tex <==
\begin{table*}[t]
\caption{Comparison of mIoU results for different methods on the \textbf{SYNTHIA$\rightarrow$Cityscapes} task. Methods marked with $^\sharp$ are based on DeepLab-v3+ \citep{chen2018encoderdecoder}, the ones with $^\dagger$ on SegFormer-B4 \citep{xie2021segformer}, whereas all the others use DeepLab-v2 \citep{deeplab2018}.}
\label{tab:synthia-cityscapes}
\centering
\begin{sc}
\begin{small}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccccccccccc}
\toprule
Method & Budget & \rot{road} & \rot{side.} & \rot{buil.} & \rot{wall*} & \rot{fence*} & \rot{pole*} & \rot{light} & \rot{sign} & \rot{veg.} & \rot{sky} & \rot{pers.} & \rot{rider} & \rot{car} & \rot{bus} & \rot{motor.} & \rot{bike} & mIoU & mIoU* \\
\midrule
Eucl. Source Only & 0\% & 64.3 & 21.3 & 73.1 & 2.4 & 1.1 & 31.4 & 7.0 & 27.7 & 63.1 & 67.6 & 42.2 & 19.9 & 73.1 & 15.3 & 10.5 & 38.9 & 34.9 & 40.3 \\
Hyper. Source Only & 0\% & 36.4 & 21.1 & 56.4 & 13.3 & 0.1 & 24.8 & 0.0 & 9.5 & 78.8 & 70.4 & 54.2 & 8.6 & 77.9 & 35.8 & 11.7 & 27.3 & 32.9 & 37.5 \\
Hyper. Source Only$^\sharp$ & 0\% & 60.5 & 27.4 & 75.2 & 13.3 & 0.3 & 31.4 & 0.0 & 23.2 & 79.3 & 68.1 & 57.8 & 18.7 & 61.3 & 27.3 & 10.3 & 23.5 & 36.1 & 41.0 \\
\midrule
% CBST \citep{zou2018unsupervised} & 68.0 & 29.9 & 76.3 & 10.8 & 1.4 & 33.9 & 22.8 & 29.5 & 77.6 & 78.3 & 60.6 & 28.3 & 81.6 & 23.5 & 18.8 & 39.8 & 42.6 & 48.9 \\
% MRKLD \citep{Zou_2019_ICCV} & 67.7 & 32.2 & 73.9 & 10.7 & 1.6 & 37.4 & 22.2 & 31.2 & 80.8 & 80.5 & 60.8 & 29.1 & 82.8 & 25.0 & 19.4 & 45.3 & 43.8 & 50.1 \\
% DPL-Dual \citep{cheng2021dual} & 87.5 & 45.7 & 82.8 & 13.3 & 0.6 & 33.2 & 22.0 & 20.1 & 83.1 & 86.0 & 56.6 & 21.9 & 83.1 & 40.3 & 29.8 & 45.7 & 47.0 & 54.2 \\
% TPLD \citep{shin2020two} & 80.9 & 44.3 & 82.2 & 19.9 & 0.3 & 40.6 & 20.5 & 30.1 & 77.2 & 80.9 & 60.6 & 25.5 & 84.8 & 41.1 & 24.7 & 43.7 & 47.3 & 53.5 \\
% Seg-Uncertainty \citep{zheng2021rectifying} & 87.6 & 41.9 & 83.1 & 14.7 & 1.7 & 36.2 & 31.3 & 19.9 & 81.6 & 80.6 & 63.0 & 21.8 & 86.2 & 40.7 & 23.6 & 53.1 & 47.9 & 54.9 \\
% ProDA \citep{zhang2021prototypical} & 87.8 & 45.7 & 84.6 & 37.1 & 0.6 & 44.0 & 54.6 & 37.0 & 88.1 & 84.4 & 74.2 & 24.3 & 88.2 & 51.1 & 40.5 & 45.6 & 55.5 & 62.0 \\
% WeakDA (point) \citep{paul2020domain} & 94.9 & 63.2 & 85.0 & 27.3 & 24.2 & 34.9 & 37.3 & 50.8 & 84.4 & 88.2 & 60.6 & 36.3 & 86.4 & 43.2 & 36.5 & 61.3 & 57.2 & 63.7 \\
% \midrule
RIPU \citep{xie2022ripu} & 2.2\% & 96.8 & 76.6 & 89.6 & 45.0 & 47.7 & 45.0 & 53.0 & 62.5 & 90.6 & \textbf{92.7} & 73.0 & 52.9 & 93.1 & 80.5 & 52.4 & 70.1 & 70.1 & 75.7 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO} (ours) & 2.2\% & \textbf{97.5} & \textbf{81.7} & \textbf{90.5} & \textbf{52.8} & \textbf{52.8} & \textbf{45.6} & \textbf{57.3} & \textbf{67.1} & \textbf{91.2} & 92.6 & \textbf{74.5} & \textbf{54.9} & \textbf{93.3} & \textbf{81.6} & \textbf{55.2} & \textbf{71.1} & \textbf{72.5} & \textbf{77.6} \\
\midrule
AADA$^\sharp$ \citep{su2020active} & 5\% & 91.3 & 57.6 & 86.9 & 37.6 & 48.3 & 45.0 & 50.4 & 58.5 & 88.2 & 90.3 & 69.4 & 37.9 & 89.9 & 44.5 & 32.8 & 62.5 & 61.9 & 66.2 \\
MADA$^\sharp$ \citep{ning2021multi} & 5\% & 96.5 & 74.6 & 88.8 & 45.9 & 43.8 & 46.7 & 52.4 & 60.5 & 89.7 & 92.2 & 74.1 & 51.2 & 90.9 & 60.3 & 52.4 & 69.4 & 68.1 & 73.3 \\
D$^2$ADA$^\sharp$ \citep{wu2022d2ada} & 5\% & 96.7 & 76.8 & 90.3 & 48.7 & 51.1 & 54.2 & 58.3 & 68.0 & 90.4 & 93.4 & 77.4 & 56.4 & 92.5 & 77.5 & 58.9 & 73.3 & 72.7 & 77.7 \\
RIPU$^\sharp$ \citep{xie2022ripu} & 5\% & 97.0 & 78.9 & 89.9 & 47.2 & 50.7 & 48.5 & 55.2 & 63.9 & 91.1 & 93.0 & 74.4 & 54.1 & 92.9 & 79.9 & 55.3 & 71.0 & 71.4 & 76.7 \\
\rowcolor[HTML]{ebebeb}
\textbf{HALO}$^\sharp$ (ours) & 5\% & \textbf{97.5} & \textbf{81.5} & \textbf{91.5} & \textbf{56.5} & \textbf{52.7} & \textbf{57.0} & \textbf{63.2} & \textbf{72.9} & \textbf{92.0} & \textbf{94.4} & \textbf{77.8} & \textbf{57.4} & \textbf{94.4} & \textbf{86.1} & \textbf{60.5} & \textbf{73.5} & \textbf{75.6} & \textbf{80.2} \\
\textbf{HALO}$^\dagger$ (ours) & 5\% & 98.3 & 86.5 & 92.6 & 61.0 & 61.5 & 60.6 & 67.6 & 76.2 & 93.2 & 94.6 & 80.8 & 58.9 & 95.0 & 85.1 & 62.7 & 75.6 & 78.1 & 82.1 \\
\midrule
Eucl. Supervised DA & 100\% & 96.7 & 77.8 & 90.2 & 40.1 & 49.8 & 52.2 & 58.5 & 67.6 & 91.7 & 93.8 & 74.9 & 52.0 & 92.6 & 70.5 & 50.6 & 70.2 & 70.6 & 75.9 \\
Hyper. Supervised DA & 100\% & 97.6 & 81.9 & 90.2 & 52.0 & 49.6 & 45.5 & 51.7 & 65.0 & 90.9 & 93.0 & 73.1 & 50.3 & 92.6 & 80.7 & 50.8 & 69.2 & 70.9 & 75.9 \\
Eucl. Supervised DA$^\sharp$ & 100\% & 97.5 & 81.4 & 90.9 & 48.5 & 51.3 & 53.6 & 59.4 & 68.1 & 91.7 & 93.4 & 75.6 & 51.9 & 93.2 & 75.6 & 52.0 & 71.2 & 72.2 & 77.1 \\
Hyper. Supervised DA$^\sharp$ & 100\% & 97.7 & 82.2 & 90.3 & 53.0 & 48.8 & 51.7 & 56.0 & 66.1 & 91.4 & 94.2 & 75.0 & 51.5 & 93.4 & 82.1 & 52.8 & 70.2 & 72.3 & 77.1 \\
Eucl. Supervised DA$^\dagger$ & 100\% &&&&&&&&&&&&&&&&& X & \\
Hyper. Supervised DA$^\dagger$ & 100\% &&&&&&&&&&&&&&&&& 77.3 & \\
\bottomrule
\end{tabular}%
}
\end{small}
\end{sc}
\end{table*}
